Incremental Reading for Question Answering

Any system which performs goal-directed continual learning must not only learn incrementally but process and absorb information incrementally. Such a system also has to understand when its goals have been achieved. In this paper, we consider these issues in the context of question answering. Current state-of-the-art question answering models reason over an entire passage, not incrementally. As we will show, naive approaches to incremental reading, such as restriction to unidirectional language models in the model, perform poorly. We present extensions to the DocQA [2] model to allow incremental reading without loss of accuracy. The model also jointly learns to provide the best answer given the text that is seen so far and predict whether this best-so-far answer is sufficient.

==> earlystop_results.tex <==
\usetikzlibrary{patterns}


\pgfplotstableread{
Context_Length Best_Performance Earlystopping(slice_size=128) Full
128   0.545600756859035   0.4640815548780488   0.46083254493850523
256   0.43103122043519393   0.5036204268292683   0.4878902554399243
384   0.019205298013245033   0.029820884146341462   0.03935666982024598
512   0.00293282876064333   0.0024771341463414634   0.008230842005676442
640   0.0012298959318826868   0.0   0.0033112582781456954
768   0.0   0.0   0.0003784295175023652
}\tableone

\begin{figure}
\begin{subfigure}[b]{0.6\textwidth}
\centering
\vspace{-25pt}
\begin{tikzpicture}
\begin{axis}[
legend cell align={left},
height=4cm, %5cm,
width=8cm,
enlarge y limits=0.05,
enlarge x limits=0.1,
ymajorgrids,
minor tick num=1,
ybar=1pt,
bar width= 5pt,
ylabel={\texttt{Frequency of examples}},
xlabel={\texttt{Consumed number of tokens}},
xtick=data,
ticklabel style = {font=\fontsize{6}{7}\selectfont},
xtick={128, 256, 384, 512, 640, 768},
xticklabels={128, 256, 384, 512, 640, 768},
symbolic x coords={128, 256, 384, 512, 640, 768},
label style = {font=\fontsize{6}{7}\selectfont, yshift=0.5ex},
legend style={
    at={(0.95,1.2),font=\fontsize{6}{7}\selectfont}
  ,legend columns=1,
  },
]
\addplot [fill=lcolor!20!lcolor, draw=lcolor!50!lcolor, pattern color = lcolor!20!lcolor,
    % pattern = north east lines
    ]table[x index=0, y index=1]{\tableone};

\addplot [fill=wcolor!20!wcolor, draw=wcolor!50!wcolor, pattern color = wcolor!20!wcolor,
    % pattern = north east lines
    ]table[x index=0,y index=2] {\tableone};

\addplot [fill=gcolor!20!gcolor, draw=gcolor!50!gcolor
    % pattern = north east lines
    ]table[x index=0,y index=3]{\tableone};
\legend{Best,Earlystopping, Full}
\end{axis}
\end{tikzpicture}
\caption{\label{fig:es_results}\fontsize{8}{8}\selectfont{Distribution of consumed length of the sequence (For the earlystopping model slice size is 128).}}
\end{subfigure}
~
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includesvg[width=\textwidth]{earlystopping.svg}
\caption{\label{fig:earlystopping}\fontsize{7}{8}\selectfont{Percent of consumed context per full context length for early stopping with slice size of 128.}}
\end{subfigure}
\caption{Earlystopping Results}
\end{figure}






==> extension.tex <==
\subsection{Greedy Prediction}
Greedy prediction, in our task if the model can predict whether a token is 
We first investigate how greedy the baseline and incremental models are in predicting the output. As an indicator of the greediness of the models we compare their performance on the partially seen context. We measure, the performance of the model at each step as we incrementally increase the context length. For the non incremental models, we treat the partial contexts as independent examples.

In order to make the model greedy in predicting the answer as soon as it can, we apply a greedy training approach. During training we decode at every slice. Thus, the total loss of the model in this case will be:


Metrics to measure greediness:

Percent of extra tokens read after answer end:
$\frac{L_{max} - answer_{end}}{L_c}$

Percent of context read to answer the question:
$\frac{L_{max}}{L_c}$

The other question is, whether the performance of the models decrease after reading too much extra tokens.


\section{Confidence Prediction and Early stopping}
There are two challenges:
first, we want the model to predict the answer as soon as it has enough information to do so.
second, we want the model to know when it knows the answer. 

Solving the second challenge has two benefits: one is for us to evaluate the effectiveness of the incremental learning strategy.
The other benefit is that it allows the model to be more efficient by avoiding to read the whole text when it already has reached its goal.

\subsection{Predicting if the answer exist}
As a simple supervised approach for teaching the model to predict its confidence, we use a classifier that is simply trained on detecting whether an answer is contained in a given context or not. We train this classifier in a multi-tasking framwork by adding an extra objective function to the QA system. Hence, at each training step, the model not only tries to predict the right answer but also predict whether the answer is in the seen context or not.

The objective function in this scenario is:

To compare the effectiveness of the models with early stopping mechanism we can use this metric:
\begin{equation}
\frac{F_e}{F_c} \times \frac{L_c}{L_e}
\end{equation}

\subsubsection{Performance of the answer exist classifier}
\section{What does the attention tell us?}
Our main motivation for studying the attention in these models is to see if we can use it as a signal to decide to stop reading. 

To see if this is at all a possible thing or not, we need to know what is the role of the attention. Is it only helping during the training process, or does it actually contain some information about where the answer is (or where the model thinks the answer is).

\todo{cite papers that study the role of attention}

In our experiments, first we show that the attention layers have a big impact on the performance of the models. \todo{cite the related papers.}

\subsection{Impact of attention layer on the performance of the plain model}
As indicated in table \ref{table:ablation_result}, removing either of the attention layers, bidirectional attention flow and self attention, leads to a significant decrease in the performance.


\subsection{Where does the model attend to?}

Now, our question is, what each of these attention layers are doing and where are they attending to. 
We could expect different roles for the attention layers. 
In the most naive case, we expect the attention to attend to where the answer is. 
In more complicated scenarios,
the attention may attend to other clues in the context for finding the answer. 
In this section, we try to explain where the attention layers are attending to with some quantific measures. Later, we train a diagnostic classifier to see if using these quantities we can predict whether an answer exist in a given context or where is the answer.

Does the model attend to where the answer is? (or where it thinks the answer is?)

How is the attention weight distributed based on where the model thinks the answer is?

How is the attention weight distributed based on where the real answer is?

Is there any relation between where the models attends to and where the answer is?

What happens if we only use the attention weights to predict the answer? what will the model attend to then? what if we supervise the attention signal to look at where the answer is?

\subsection{What happens to attention in the sliced DocQA}
Attention distribution over slices



Comparative Analysis of QA on Squad: e.g. different error types.
https://arxiv.org/pdf/1806.06972.pdf
